Compute Only Once: UG-Separation for Efficient Large Recommendation Models

Driven by scaling laws, recommender systems increasingly rely on larger-scale models to capture complex feature interactions and user behaviors, but this trend also leads to prohibitive training and inference costs. While long-sequence models can reuse user-side computation through KV Caching, such reuse is difficult in TokenMixer-based dense feature interaction architectures, where user and group features are deeply entangled and mixed-up across layers. In this work, we present User-Group Separation (UG-Sep), an industrial large-scale framework that enables user-side computation reusable in TokenMixer-based dense interaction models for the first time. UG-Sep explicitly disentangles user-side and item-side information flows within token-mixing layers, ensuring that a subset of tokens preserves purely user-side representations across layers. This design allows the corresponding per-token computations to be reused across multiple samples, significantly reducing redundant inference cost. To compensate for the potential expressive capacity loss induced by masking, we further propose an Information Compensation strategy that adaptively reconstructs suppressed user-item interactions. Moreover, as UG-Sep substantially reduces user-side FLOPs and exposes memory-bound components, we incorporate W8A16 (8-bit weight, 16-bit activation) weight-only quantization to alleviate memory bandwidth bottlenecks and achieve additional acceleration. We conduct extensive offline evaluations and large-scale online A/B experiments at ByteDance to validate the effectiveness of UG-Sep. Results show that UG-Sep reduces inference latency by up to 20% without causing adverse changes to online user experience and commercial metrics on multiple influential business scenarios compared to TokenMixer at ByteDance, including Douyin Feed Recommendation, Hongguo Feed Recommendation, Chuanshanjia Ads, and Qianchuan Ads.

==> old_UI.tex <==
% %%
% %% This is file `sample-sigconf.tex',
% %% generated with the docstrip utility.
% %%
% %% The original source files were:
% %%
% %% samples.dtx  (with options: `all,proceedings,bibtex,sigconf')
% %% 
% %% IMPORTANT NOTICE:
% %% 
% %% For the copyright see the source file.
% %% 
% %% Any modified versions of this file must be renamed
% %% with new filenames distinct from sample-sigconf.tex.
% %% 
% %% For distribution of the original source see the terms
% %% for copying and modification in the file samples.dtx.
% %% 
% %% This generated file may be distributed as long as the
% %% original source files, as listed above, are part of the
% %% same distribution. (The sources need not necessarily be
% %% in the same archive or directory.)
% %%
% %%
% %% Commands for TeXCount
% %TC:macro \cite [option:text,text]
% %TC:macro \citep [option:text,text]
% %TC:macro \citet [option:text,text]
% %TC:envir table 0 1
% %TC:envir table* 0 1
% %TC:envir tabular [ignore] word
% %TC:envir displaymath 0 word
% %TC:envir math 0 word
% %TC:envir comment 0 0
% %%
% %% The first command in your LaTeX source must be the \documentclass
% %% command.
% %%
% %% For submission and review of your manuscript please change the
% %% command to \documentclass[manuscript, screen, review]{acmart}.
% %%
% %% When submitting camera ready or to TAPS, please change the command
% %% to \documentclass[sigconf]{acmart} or whichever template is required
% %% for your publication.
% %%
% %%
% \documentclass[sigconf]{acmart}
% \usepackage{mathtools}
% \usepackage{subcaption}
% \usepackage{float}
% \usepackage{stfloats}
% \usepackage{makecell}
% % \usepackage{mathtools}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{multirow}
% \usepackage[utf8]{inputenc}

% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     Bib\TeX}}}

% %% Rights management information.  This information is sent to you
% %% when you complete the rights form.  These commands have SAMPLE
% %% values in them; it is your responsibility as an author to replace
% %% the commands and values with those provided to you when you
% %% complete the rights form.
% \setcopyright{acmlicensed}
% \copyrightyear{2025}
% \acmYear{2025}
% \acmDOI{XXXXXXX.XXXXXXX}
% %% These commands are for a PROCEEDINGS abstract or paper.
% \acmConference[Conference acronym 'XX]{Make sure to enter the correct
%   conference title from your rights confirmation email}{June 03--05,
%   2025}{Woodstock, NY}
% %%
% %%  Uncomment \acmBooktitle if the title of the proceedings is different
% %%  from ``Proceedings of ...''!
% %%
% %%\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
% %%  June 03--05, 2018, Woodstock, NY}
% \acmISBN{978-1-4503-XXXX-X/2025/06}


% %%
% %% Submission ID.
% %% Use this when submitting an article to a sponsored event. You'll
% %% receive a unique submission ID from the organizers
% %% of the event, and this ID should be used as the parameter to this command.
% %%\acmSubmissionID{123-A56-BU3}

% %%
% %% For managing citations, it is recommended to use bibliography
% %% files in BibTeX format.
% %%
% %% You can then either use BibTeX with the ACM-Reference-Format style,
% %% or BibLaTeX with the acmnumeric or acmauthoryear sytles, that include
% %% support for advanced citation of software artefact from the
% %% biblatex-software package, also separately available on CTAN.
% %%
% %% Look at the sample-*-biblatex.tex files for templates showcasing
% %% the biblatex styles.
% %%

% %%
% %% The majority of ACM publications use numbered citations and
% %% references.  The command \citestyle{authoryear} switches to the
% %% "author year" style.
% %%
% %% If you are preparing content for an event
% %% sponsored by ACM SIGGRAPH, you must use the "author year" style of
% %% citations and references.
% %% Uncommenting
% %% the next command will enable that style.
% %%\citestyle{acmauthoryear}


% %%
% %% end of the preamble, start of the body of the document source.
% \begin{document}

% %%
% %% The "title" command has an optional parameter,
% %% allowing the author to define a "short title" to be used in page headers.
% % \title{UI-Seq: Making User-Side Computation Reusable in Recommender System}
% \title{RankMixer-v2: Separable Feature Interaction for \\Large-Scale Recommendation}


% \author{Hui Lu*}
% \thanks{*These authors contributed equally.}
% \email{luhui.xx@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Hangzhou}
%   \country{China}
% }

% \author{Zheng Chai*}
% % \authornote{Corresponding Author.}
% \email{chaizheng.cz@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Hangzhou}
%   \country{China}
% }

% \author{Shipeng Bai*}
% % \authornote{Corresponding Author.}
% \email{baishipeng@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Hangzhou}
%   \country{China}
% }

% \author{Hao Zhang*}
% % \authornote{Corresponding Author.}
% \email{zhanghao.229@bytedance.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Shanghai}
%   \country{China}
% }

% \author{Zhifang Fan*}
% % \authornote{Corresponding Author.}
% \email{fanzhifangfzf@gmail.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Shanghai}
%   \country{China}
% }

% \author{Yingwen Wu}
% % \authornote{Corresponding Author.}
% \email{wu.yingwen@bytedance.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Shanghai}
%   \country{China}
% }

% \author{Bingzheng Wei}
% % \authornote{Corresponding Author.}
% \email{weibingzheng@bytedance.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Beijing}
%   \country{China}
% }

% \author{Xiang Sun}
% % \authornote{Corresponding Author.}
% \email{sunxiang.0@bytedance.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Beijing}
%   \country{China}
% }

% \author{Ziyan Gong}
% % \authornote{Corresponding Author.}
% \email{gongziyan@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Hangzhou}
%   \country{China}
% }

% \author{Tianyi Liu}
% % \authornote{Corresponding Author.}
% \email{liutianyi.2024@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Beijing}
%   \country{China}
% }

% \author{Hua Chen}
% % \authornote{Both authors contributed equally to this research.}
% \email{chenhua.2468@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Shanghai}
%   \country{China}
% }

% \author{Deping Xie}
% % \authornote{Both authors contributed equally to this research.}
% \email{deping.xie@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{San Jose}
%   \country{USA}
% }

% \author{Zhongkai Chen}
% % \authornote{Both authors contributed equally to this research.}
% \email{chenzhongkai.666@bytedance.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Hangzhou}
%   \country{China}
% }

% \author{Zhiliang Guo}
% % \authornote{Both authors contributed equally to this research.}
% \email{guozhiliang@bytedance.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Beijing}
%   \country{China}
% }

% \author{Qiwei Chen}
% \email{chenqiwei05@gmail.com}
% \affiliation{%
%   \institution{ByteDance}
%   \city{Shanghai}
%   \country{China}
% }

% \author{Yuchao Zheng\textsuperscript{†}}
% \thanks{\textsuperscript{†}Corresponding Author.}
% \email{zhengyuchao.yc@bytedance.com}
% \affiliation{%
%   \institution{ByteDance AML}
%   \city{Hangzhou}
%   \country{China}
% }



% %%
% %% The "author" command and its associated commands are used to define
% %% the authors and their affiliations.
% %% Of note is the shared affiliation of the first two authors, and the
% %% "authornote" and "authornotemark" commands
% % %% used to denote shared contribution to the research.

% % \author{Zheng Chai*}
% % \thanks{*These authors contributed equally.}
% % \thanks{\textsuperscript{†}Corresponding Author.}
% % % \authornote{Corresponding Author.}
% % \email{chaizheng.cz@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Hangzhou}
% %   \country{China}
% % }

% % \author{Qin Ren*}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{renqin.97@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Xijun Xiao*}
% % \email{xiaoxijun@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Huizhi Yang*}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{yanghuizhi@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Bo Han*}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{hanbo.1990@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Shanghai}
% %   \country{China}
% % }

% % \author{Sijun Zhang}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{zhangsijun.randyz@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Di Chen}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{chendi.666@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Hui Lu}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{luhui.xx@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Hangzhou}
% %   \country{China}
% % }

% % \author{Wenlin Zhao}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{zhaowenlin@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Lele Yu}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{yulele@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{San Jose}
% %   \country{USA}
% % }

% % \author{Xionghang Xie}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{xiexionghang@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Shiru Ren}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{zhangyunqi.90@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Xiang Sun}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{sunxiang.0@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Yaocheng Tan}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{tanyaocheng@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % % \author{Yunqi Zhang}
% % % % \authornote{Both authors contributed equally to this research.}
% % % \email{zhangyunqi.90@bytedance.com}
% % % \affiliation{%
% % %   \institution{ByteDance}
% % %   \city{Beijing}
% % %   \country{China}
% % % }


% % \author{Peng Xu}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{xupeng@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{San Jose}
% %   \country{USA}
% % }


% % \author{Yuchao Zheng\textsuperscript{†}}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{zhengyuchao.yc@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Di Wu}
% % % \authornote{Both authors contributed equally to this research.}
% % \email{di.wu@bytedance.com}
% % \affiliation{%
% %   \institution{ByteDance}
% %   \city{Beijing}
% %   \country{China}
% % }

% % \author{Ben Trovato}
% % \authornote{Both authors contributed equally to this research.}
% % \email{trovato@corporation.com}
% % \orcid{1234-5678-9012}
% % \author{G.K.M. Tobin}
% % \authornotemark[1]
% % \email{webmaster@marysville-ohio.com}
% % \affiliation{%
% %   \institution{Institute for Clarity in Documentation}
% %   \city{Dublin}
% %   \state{Ohio}
% %   \country{USA}
% % }

% % \author{Lars Th{\o}rv{\"a}ld}
% % \affiliation{%
% %   \institution{The Th{\o}rv{\"a}ld Group}
% %   \city{Hekla}
% %   \country{Iceland}}
% % \email{larst@affiliation.org}

% % \author{Valerie B\'eranger}
% % \affiliation{%
% %   \institution{Inria Paris-Rocquencourt}
% %   \city{Rocquencourt}
% %   \country{France}
% % }

% % \author{Aparna Patel}
% % \affiliation{%
% %  \institution{Rajiv Gandhi University}
% %  \city{Doimukh}
% %  \state{Arunachal Pradesh}
% %  \country{India}}

% % \author{Huifen Chan}
% % \affiliation{%
% %   \institution{Tsinghua University}
% %   \city{Haidian Qu}
% %   \state{Beijing Shi}
% %   \country{China}}

% % \author{Charles Palmer}
% % \affiliation{%
% %   \institution{Palmer Research Laboratories}
% %   \city{San Antonio}
% %   \state{Texas}
% %   \country{USA}}
% % \email{cpalmer@prl.com}

% % \author{John Smith}
% % \affiliation{%
% %   \institution{The Th{\o}rv{\"a}ld Group}
% %   \city{Hekla}
% %   \country{Iceland}}
% % \email{jsmith@affiliation.org}

% % \author{Julius P. Kumquat}
% % \affiliation{%
% %   \institution{The Kumquat Consortium}
% %   \city{New York}
% %   \country{USA}}
% % \email{jpkumquat@consortium.net}

% %%
% %% By default, the full list of authors will be used in the page
% %% headers. Often, this list is too long, and will overlap
% %% other information printed in the page headers. This command allows
% %% the author to define a more concise list
% %% of authors' names for this purpose.
% \renewcommand{\shortauthors}{xx et al.}

% %%
% %% The abstract is a short summary of the work to be presented in the
% %% article.
% \begin{abstract}
% Driven by scaling laws, recommender systems increasingly rely on larger-scale models to capture complex feature interactions and user behaviors, but this trend also leads to prohibitive training and inference costs. While long-sequence models (e.g., LONGER) can reuse user-side computation through KV Caching, such reuse is difficult in dense feature interaction architectures (e.g., RankMixer), where user and item features are deeply entangled across layers. In this work, we propose \textbf{RankMixer-v2}, a novel framework that enables \textbf{User–Item Separation (UI-Sep)} and makes user-side computation reusable in dense interaction models for the first time. UI-Sep introduces a masking mechanism that explicitly disentangles user-side and item-side information flows within token-mixing layers, ensuring that a subset of tokens preserves purely user-side representations across layers. This design allows the corresponding per-token computations to be reused across multiple samples, significantly reducing redundant inference cost. To compensate for the potential expressive capacity loss induced by masking, we further propose an Information Compensation strategy that adaptively reconstructs suppressed user–item interactions. Moreover, as UI-Sep substantially reduces user-side FLOPs and exposes memory-bound components, we incorporate W8A16 (8-bit weight, 16-bit activation) weight-only quantization to alleviate memory bandwidth bottlenecks and achieve additional acceleration. We conduct extensive offline evaluations and large-scale online A/B experiments at ByteDance to validate the effectiveness of UI-Sep. Results show that UI-Sep reduces inference latency by up to 20\% without causing adverse changes to online user experience and commercial metrics on multiple business scenarios, including Douyin recommendation, Hongguo recommendation, Chuanshanjia Ads and Qianchuan Ads.



% % For example, in Douyin’s recommendation system, UI-Sep reduces inference latency by up to 20\% without causing adverse changes to online user experience and commercial metrics, demonstrating its practicality and robustness for large-scale industrial recommender systems.
% \end{abstract}


% % Transformer-based framework optimized for end-to-end ultra-long sequence modeling with industrial-level scalability.

% %%
% %% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
% %% Please copy and paste the code instead of the example below.
% %%

% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>00000000.0000000.0000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Information systems~Recommender systems}

% %%
% %% Keywords. The author(s) should pick words that accurately describe
% %% the work being presented. Separate the keywords with commas.
% \keywords{Large Recommender Model, Industrial Recommenders, Scaling Law}

% %% A "teaser" image appears between the author and affiliation
% %% information and the body of the document, and typically spans the
% %% page.
% % \begin{teaserfigure}
% %   \includegraphics[width=\textwidth]{sampleteaser}
% %   \caption{Seattle Mariners at Spring Training, 2010.}
% %   \Description{Enjoying the baseball game from the third-base
% %   seats. Ichiro Suzuki preparing to bat.}
% %   \label{fig:teaser}
% % \end{teaserfigure}

% % \received{20 February 2007}
% % \received[revised]{12 March 2009}
% % \received[accepted]{5 June 2009}

% %%title
% %% This command processes the author and affiliation and title
% %% information and builds the first copypart of the formatted document.
% \maketitle

% \section{Introduction}

% %background
% Propelled by the scaling law, Recommender System (RS) have continuously expanded in terms of parameter scale, training data volume, and computational cost, with widespread deployment in core processes such as recall\cite{lian2020lightrec,diaz2025recall,li2024harnessing,altosaar2021rankfromsets}, ranking\cite{zehlike2022fairness,deng2025onerec,bao2025bi,jiang2025beyond}, and multitask learning\cite{wang2023towards,zhang2025optimizing}  in recent years. Such larger models can capture more complex feature interaction user behavior patterns and long-term preferences, significantly improving recommendation performance.
% However, this growth has led to an exponential increase in training and inference costs, posing a critical challenge for model deployment.

% Currently, the main methods for scaling recommender model can be divided into two categories: long sequence modeling\cite{chai2025longer,deng2025onerec,xu2025climber,chai2022user} and dense scaling up\cite{zhu2025rankmixer,zhang2024wukong}.
% %sequence
% In long sequence modeling scenarios, samples generated by the same user at different time points typically share substantial portions of their historical behavior sequences. Motivated by this feature, User-Level Training\cite{zhai2024actions, chai2025longer} is widely employed during the training phase, wherein samples belonging to the same user within a specified temporal window are aggregated and optimized jointly. This aggregation enables computation reuse over shared sequence prefixes, leading to a substantial improvement in overall training efficiency. During the inference phase, KV-Cache mechanisms (e.g., M-Falcon\cite{zhai2024actions}) are used to cache the representations of the user-side historical sequences. This allows for the reuse of prefix computation results when processing each new candidate item, significantly reducing inference costs and latency. 

% %dense
% However, such aggregation strategies are difficult to apply in dense feature interaction scenarios. Module like RankMixer\cite{zhu2025rankmixer} and MLP-Mixer\cite{li2025research,gong2025pyramid,qi2025mtmixatt}, which involve deep cross-interaction between user-side and candidate-side features, perform intricate feature fusion at each layer through mechanisms such as channel mixing, self-attention, or nonlinear interactions. Thus, user-side features cannot be treated as independent prefixes that can be cached and reused. Whenever the candidate item changes, all cross-layer fusion computations must be recomputed, leading to a significant item dependency in the inference process. As a result, with the continuous increase in model width and depth, the inference overhead in dense scaling rises rapidly with model size, becoming a critical bottleneck for further expansion and industrial deployment of large-scale Recommender System.

% % \footnote{“Good” denotes the item-side entity in recommendation system, such as a product, advertisement, video, or content that interacts with users.}

% To address the aforementioned limitations, we introduce User–Item Separation(UI-Sep), the first technique designed to enable the reuse of user-side representations within architectures such as RankMixer and MLP-Mixer, which substantially reduces redundant computations and inference latency in dense scaling scenarios. 


% %mask
% Specifically, we \textbf{first} introduce a novel masking mechanism that explicitly disentangles the information flows of the user side and item side within the model. This mechanism guarantees that a designated subset of tokens retains purely user-side information even after passing through arbitrary layer transformations, thereby enabling their associated per-token FFN\cite{zhu2025rankmixer} computations to be shared across multiple samples via User-Level aggregation. 
% %information compresation
% \textbf{Second}, since the imposed masking inevitably leads to partial information loss and may diminish the model’s expressive capacity, we propose an Information Compensation strategy that adaptively reconstructs the suppressed or missing interactions between user and candidate features, ensuring that the model preserves robust predictive performance while benefiting from substantial computational savings.
% %W8A16
% \textbf{Last but not least}, with the adoption of UI-Sep, the FLOPs on the U-side are substantially reduced, causing certain components in RankMixer to become memory-bound. To mitigate this emerging memory bottleneck, we incorporate the W8A16 quantization\cite{kim2025zero,yashaswini2025non} technique, which effectively alleviates memory pressure and enables additional acceleration. Extensive offline and online experiments have validated the effectiveness of our approach. For example, in the production deployment of Douyin's recommendation system, UI-sep has reduced inference latency by 20\% while maintaining stable online metrics. This demonstrates the feasibility and stability of the method in real-world production environments. In summary, our contributions are as follows:
% \begin{itemize}
%     \item We introduce RankMixer-v2, the first technique specifically designed for separable feature interaction in large recommendation models. By combining a novel masking mechanism, an information compensation strategy, and a W8A16 quantization, RankMixer-v2 isolates user–item information flows, and thus enables effective reuse of user-side representations that were previously inseparable in dense models.
    
%     \item The core UI-Sep mechanism is highly general and can be readily integrated into a wide range of interaction architectures, including MLP-Mixer variants, Transformer-based structures, and other dense interaction models, without requiring modifications to their fundamental design principles.
    
%     \item Extensive empirical studies conducted both on large-scale industrial datasets and through online A/B testing on multiple high-traffic platforms at ByteDance demonstrate the practical value of the method.
% \end{itemize}




% \section{Related Work}
% We describe related work in two parts: long-sequence modeling,  and large-scale feature interaction models.

% % dense scale up model.


% \subsection{Long-Sequence Modeling}
% Modeling long-term user behavior sequences has been a central topic in recommender systems. Early approaches employ RNN and CNN-based architectures\cite{zhou2018deep, zhou2019deep, chang2021sequential, zhou2019deep,zhou2020can} to capture sequential dependencies. Besides, multi-domain\cite{chai2025adaptive,chang2023pepnet}, multi-interest\cite{li2019multi,chai2022user}, and sequence denoising methods\cite{shin2024attentive,chen2022denoising} are extensively approached for different aspects in modeling user preferences. As recommender systems continue to scale, several studies investigate the scaling behavior of sequential models. Actions Speak Louder than Words\cite{zhai2024actions} demonstrates that large-scale sequential transducers, even at trillion-parameter scale, can capture complex user behavior patterns for generative recommendation. Similarly, Zivic et al.\cite{zivic2024scaling} analyzes how Transformer-based sequential models benefit from scaling in model size and sequence length. To support industrial deployment, system-oriented solutions such as LONGER\cite{chai2025longer} focus on scaling up long-sequence modeling in production environments by optimizing data pipelines and training strategies, enabling practical use of ultra-long user histories.

% However, the introduction of ultra-long user behavior sequences also brings substantial computational challenges. As sequence length increases, the computational complexity and memory overhead during both training and inference grow rapidly, becoming a critical bottleneck that limits further scaling and practical deployment of sequential models. To address this issue, recent studies have explored solutions from the perspective of computation reuse and system-level optimization. For example, HSTU\cite{zhai2024actions} leverages shared user behavior sequences to achieve efficient training and inference, thereby highlighting the importance of sequence-level computation reuse in extreme-scale generative recommendation settings. LONGER\cite{chai2025longer} explicitly targets the efficiency challenges of long-sequence modeling by adopting user-level sequence organization and system optimizations, enabling scalable training with ultra-long user histories while significantly reducing redundant computation. Similarly, Zivic et al. \cite{zivic2024scaling} systematically studies how Transformer-based sequential recommenders scale in practice and emphasizes user-level sample organization and prefix sharing as essential techniques for improving training efficiency at scale. UniRec\cite{xie2024unifiedssr} proposes a unified framework for sequential recommendation that reuses user behavior sequences across different recommendation tasks and samples, thereby substantially improving training and inference efficiency. Overall, these studies consistently demonstrate that user-level sequence–centric organization and prefix reuse mechanisms are key factors in accelerating sequential recommendation models, laying a solid foundation for efficient scaling in long-sequence scenarios.


% \subsection{Dense scaling up}

% Beyond sequence-based approaches, dense interaction models have gained increasing attention due to their strong expressive power. Such models perform deep cross-interaction between user-side and item-side features at every block, enabling fine-grained feature fusion. 
% Representative architectures include cross-attention–based Transformers~\cite{vaswani2017attention}, MLP-Mixer–style token mixing models~\cite{tolstikhin2021mlp,zhu2025rankmixer}.

% Despite their effectiveness, dense interaction models exhibit strong item dependency: user-side representations are repeatedly fused with candidate-side features throughout the network. As a result, user representations cannot be isolated as reusable prefixes. Whenever the candidate item changes, all cross-layer fusion computations must be recomputed, causing inference cost to scale linearly with the number of candidates. As model width and depth continue to increase, this property leads to rapidly growing inference overhead, becoming a major bottleneck for dense scaling in industrial recommender systems. To the best of our knowledge, existing work has not provided a general mechanism to enable user-side computation reuse in dense interaction architectures without fundamentally modifying their core model structures.


% \begin{figure*}[t]
%     \centering
%         \centering
%         \includegraphics[width=1\linewidth ]{image/tokenmixer.pdf}
%         \caption{RankMixer-v2 Layer with UI-Sep.}\label{fig:mixup}
% \end{figure*}



% \section{Method}
% \subsection{Separatation of UI Token}
% In existing feature-interaction modules (e.g., RankMixer\cite{zhu2025rankmixer,qi2025mtmixatt,zhang2025billion}, Self-Attention\cite{vaswani2017attention,yu2025hhft}), the input tokens typically encode a mixture of both U-side and I-side information. However, UI-Sep requires that the inputs to these interaction modules be cleanly separated into user-side and item-side representations. To satisfy this requirement, we first decouple the U-side and I-side features at the bottom layers of the network. Correspondingly, the feature-extraction modules (e.g., SENet\cite{chen2025squeeze},DCN\cite{wang2017deep}) are split into two branches: one dedicated to extracting U-side features and the other to extracting I-side features. Also, for modules whose structural complexity prevents a clean separation between U-tokens and I-tokens, we treat their outputs as I-side features. As a result, tokens that only contain purely user-related information are designated as U-tokens, whereas tokens that contain both user and item information are categorized as I-tokens. This architectural arrangement ensures that the inputs to subsequent feature-interaction modules can be rigorously partitioned into U-tokens and I-tokens, as illustrated in Figure~\ref{fig:mixup}.


% \subsection{Separation of UI Interaction}
% Based on the above decomposition, the inputs to the feature-interaction module have now been separated into U-tokens and I-tokens. To ensure the reusability of U-side outputs, it is essential to prevent any I-side information from being exposed to or entangled with the U-side. In the following sections, we describe how to design an appropriate mask for RankMixer\cite{zhu2025rankmixer} to guarantee the independence of U-side information.

% % \subsection{RankMixer with UI-Sep}
% We use the RankMixer architecture \cite{zhu2025rankmixer}, which has two core components: (1) Multi-Head Token Mixing layer, and (2) Per-Token FeedForward Network (PFFN) layer:
% \begin{align}
%     P_{k-1} &= LN\bigl(Mixup
%     (X_{k-1}) \bigr) \\
%     X_{k} &= LN\bigl(PFFN(P_{k-1}) + X_{k-1}\bigr)
% \end{align}

% \noindent where $LN(\cdot)$ is the layer normalization function, $Muxup(\cdot)$ and
% $PFFN(\cdot)$ are the multi-head Token Mixing module and the pertoken FFN module,
% $ X_k \in \mathbb{R}^{T \times D} $ is the output of the $k-th$ RankMixer
% block, $T$ is the token number and $D$ is the hidden
% dimension of the model. 
% With UI separation, $X$ can be denote as follow:
% \begin{equation}
%     X = Concat(x_{u^0}, x_{u^1}, \cdots, x_{u^{n-1}}, x_{i^0}, x_{i^1}, \cdots, x_{i^{m-1}})
% \end{equation}
%  where $x_u$ is the U-side token, $x_i$ is the I-side token, $n$ is the number of U token, and $m$ is the number of $I-token$, where $m+n = T$. A core component of the RankMixer is the mixup module, which splits and transposes the input tokens to enable thorough interaction across token dimensions. It first split the each token with $H$ head:
%  \begin{align}
%      Split(x_{u^0})=(x_{u^0}^0, x_{u^0}^1,\cdots, x_{u^0}^{H-1})
%  \end{align}
 
%  Let $D'$ denote the dimension of each head, with $D' = D / H$. Accordingly, $x_{u^0}^{H-1} \in \mathbb{R}^{1 \times D'} $ for each head $h$. We then concat the splited head to get the new token $L$:

 
% \begin{align}
%         \label{eq:uginformation}
%      L^h = Concat(x_{u^0}^h, x_{u^1}^h,\cdots,x_{i^{T-1}}^h), h \in [0,H-1]
%  \end{align}
% $L^h \in \mathbb{R}^{1 \times D'*T}$ contains both U-side and I-side information. After the above transformation, $H$ new tokens are produced. By concatenating these tokens, we obtain the output of the mixup module.
%  \begin{align}
%        Mixup(X) = Concat(L^0,L^1,\cdots, L^{H-1})
%  \end{align}
 
% At this stage, we assume that among the newly generated tokens, the first $c_u$ are U-tokens and the remaining $c_i$ are I-tokens, where $c_u + c_i = H$.  \textbf{To ensure that the computation results on the U-side can be reused, we must guarantee that the $c_u$ U-tokens has no I-side information}. To achieve this, we first introduce a masking mechanism that removes any I-side signals from these user tokens. The mask can be formula as follow:

% \begin{align}
%     mask_{i,j} = 
% \begin{cases}
% 0, \quad i<c_u,\quad j>n*D', \quad  \\
% 1, \quad otherwise
% \end{cases}
% \end{align}
% where $i \in [0, H-1],\quad j\in[0, T*D']$.
% As shown in Fig.\ref{fig:mixup}, we can remove the I-side information from U-token through the following equation:
% \begin{equation}
%     X_{masked} = Mixup(X) * broadcast(mask)
% \end{equation}

% Thus, after the mask transformation, we obtain a new set of tokens, where the first $c_u$
% tokens are designated as U-tokens and contain no I-side information. The remaining tokens correspond to I-tokens.
% %more complex
% The other component of the RankMixer is the PFFN layer, which we decompose into two parts: a reusable PerToken-AFFN and a non-reusable PerToken-AFFN. As shown in Fig.\ref{fig:mixup}, as U-side tokens are irrelevant to different candidate items in online serving, and thus these tokens are processed through the reusable PerToken-AFFN, while I-side tokens are passed through the non-reusable counterpart. This design ensures that the computation associated with U-side tokens only needs to be performed once for each user in serving, enabling the reduction from $\mathcal{O}(C)$ to $\mathcal{O}(1)$ for the U-token part, where $C$ is the number of candidate items in ranking stage of industrial recommenders.
% % efficient reuse across different inference settings.

% \subsection{UI-Sep with Separated Residual}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth,clip]{image/ug-resi.pdf}
%     \caption{UI-Sep with Separated Residual}
%     \label{fig:ug-resi}
% \end{figure}
% When the number of U-side tokens in the input $X$, denoted by $n$, and the number of I-side tokens, denoted by $m$, are respectively equal to the numbers of U-side and I-side tokens after the Mixup operation, denoted by $C_u$ and $C_I$, a direct residual connection can be applied. As a result, U-side information remains isolated, ensuring strict preservation of U-side independence.

%  However, in practical applications, a pyramidal design-where the number of output tokens is smaller than that of the input—is often used to achieve higher computational efficiency, typically accompanied by residual connections. Such designs are commonly applied in deeper layers: lower layers employ the standard RankMixer to perform full cross-token interaction, while upper layers adopt the pyramidal structure to improve parameter and computational efficiency. Consequently, when the UI-Sep mechanism is incorporated into a pyramidal RankMixer, the number of input U-side tokens $n$ is no longer equal to the number of mixup output U-token $C_u$, which complicates the design of the residual pathway, as it must strictly prevent I-side features from being propagated into U-side tokens.

% One possible solution is inspired by the cross-attention mechanism (see Fig.\ref{fig:ug-resi}). Specifically, the output of the Mixup followed by the FFN is used as the query, and a cross-attention operation is performed over the input tokens of the current mixer layer. The resulting output is then added back to the Mixup output as a residual connection. To maintain UI separation under this design, an additional UI mask must be incorporated into the cross-attention computation. This approach has the benefit of eliminating the constraint that the input and output tokens must maintain a fixed U/G proportion. 

% % However, it also introduces additional complexity into the residual design, and careful handling is required to ensure that U-side independence is preserved.


% \subsection{Information Compensation}
% As illustrated in Fig.\ref{fig:inforation Compensation}, the UI-separation masking operation inevitably removes part of the U-side head information along the dimensional axes associated with I-side tokens, which introduces a certain degree of information loss. Empirically, we observe that when the proportions of U-side and I-side tokens remain close to their original allocation, this loss has a negligible impact on model performance. A plausible explanation is that the masked dimensions account for only a small fraction of the overall representation, and the residual connections are able to partially compensate for the missing information.

% However, further experiments show that when the proportion of U-side tokens becomes significantly larger than that of I-side tokens (e.g., ratios of U:I become 2:1, 3:1, or even 5:1), model performance degrades substantially. In such cases, the masked I-related dimensions occupy a much larger portion of the representation space, and residual connections alone are no longer sufficient to recover the lost information.

% To address this issue, we introduce an information compensation mechanism. The key idea is to explicitly inject U-side information back into the I-side representations after UI masking.
% Formally, let $U \in \mathbb{R}^{C_u \times d}$ denote the U-side token representations after the Mixup operation and UI masking, $I \in \mathbb{R}^{C_I \times d}$ denote the corresponding I-token representations. We first project the U-side representations into the same feature dimension as the I-side tokens:
% \begin{equation}
% \hat{U} = \mathrm{Proj}(U)
% \end{equation}
% where $\mathrm{Proj}(\cdot)$ is a learnable linear projection.
% The projected U-token are then added to the I-tokens to compensate for the masked information:

% \begin{equation}
% I_{\mathrm{comp}} = I + \hat{U}
% \end{equation}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{image/information_compensation.pdf}
%     \caption{Information Compensation}
%     \label{fig:inforation Compensation}
% \end{figure}

% As shown in Fig.\ref{fig:inforation Compensation}, this operation can be interpreted as transferring the preserved U-side information back to the I-side tokens through a lightweight projection-and-addition pathway. By doing this, the model restores the missing contextual information caused by UI masking while still maintaining strict U-side independence, since no I-side information is injected into U-side tokens. This information compensation mechanism is particularly important in pyramidal RankMixer settings, where the imbalance between U-side and I-side token proportions becomes more pronounced.
% \begin{algorithm}[b]
% \caption{In-request U-side Caching}
% \label{al:algo}
% \begin{algorithmic}[1]
% \State \textbf{Input:} candidate\_size\_tensor $\in \mathbb{R}^{M}$, \; INPUT\_U, INPUT\_I $\in \mathbb{R}^{N}$
% \State \textbf{Output:} OUTPUT\_U
% \Statex

% \State Offset $\gets$ \textsc{Cumsum}(candidate\_size\_tensor)
% \State Unique\_U $\gets$ \textsc{Gather}(INPUT\_U, Offset)
% \State Unique\_U $\gets$ \textsc{RankMixer}(Unique\_U)
% \State OUTPUT\_U $\gets$ \textsc{Repeat}(Unique\_U, candidate\_size\_tensor)

% \end{algorithmic}
% \end{algorithm}


% \subsection{W8A6 Quantizaion Method}
% % UI separation enables computational acceleration in both the training and serving stages. However, during training, such acceleration can only be realized when the training data are organized as user-level aggregations (e.g., M-Falcon \cite{zhai2024actions}), enabling reuse of U-side computations across samples. In contrast, in the serving stage of recommendation and advertising systems, U-side information is naturally aggregated within the system architecture. Consequently, no modification to the serving pipeline is required to cache U-side computations, allowing acceleration to be obtained directly. Therefore, in the following sections, we focus primarily on the serving process.

% In the serving stage, we cache the U-side computations. As shown in Algorithm \ref{al:algo}, for each candidate item, the cached U-side results can be directly reused, leading to a theoretical speedup proportional to the number of candidates. The expected FLOPS acceleration can be approximated by the following formulation:



% \begin{align}
%     ratio = \frac{c_u}{c_{u}+c_{I}}
%     \label{eq: flops}
% \end{align}


% As shown in Eq.~\ref{eq: flops}, the FLOPs are substantially reduced by 50\%, if $c_u$ is equal to $c_I$. However, the forward latency does not decrease proportionally, as the computation is bounded by memory throughput rather than compute operations. To address this bottleneck, we propose a 8-bit weight and 16-bit activation strategy (W8A16), which significantly reduces memory traffic and leads to noticeable latency improvements.

% \textbf{W8A16} is a weight-only quantization method. In memory-bound regimes, the dominant performance bottleneck arises not from arithmetic operations but from the high memory bandwidth required to load large parameter matrices. Weight-only quantization provides an effective solution by reducing the bit-width of weights while keeping activations in higher precision. By storing weights in 8-bit (FP8) format and dequantizing them on-chip during computation, the required memory traffic is reduced by up to 4× compared to FP32 and 2× compared to BF16 storage. Because activations remain in 16-bit precision (A16), the expressiveness and numerical stability of the forward pass are preserved, making the scheme compatible with large-scale recommendation models and high-throughput serving scenarios.
% The computational overhead introduced by dequantization is negligible relative to the savings in memory traffic. As a result, W8A16 quantization substantially alleviates memory bottlenecks and yields pronounced latency improvements, especially in workloads with small batch sizes or models with UI Separate, where weight loading dominates execution time.




% \subsection{Generalizing UI-Sep to Standard Attention}
% %Another important module widely used across various domains is the attention mechanism.
% We extend UI separation from RankMixer-based interaction modules to Attention-based architectures, demonstrating its generality across different feature interaction paradigms.
% To enable U-side computation reuse within attention, we develop a UI-masked attention variant that enforces U-side independence while preserving the expressiveness of the original formulation:
% The standard attention computation is defined as:
% \begin{equation}
%     Attn(X)={softmax}\!\left(
%     \frac{QK^{\top}}{\sqrt{d}}\right)V 
% \end{equation}
% where,
% \begin{align}
% Q = XW_{Q}, 
% K = XW_{K}, 
% V = XW_{V}.
% \end{align}
% Under the UI framework, the input token sequence is partitioned into U-side and I-side tokens. 
% Accordingly, the query and key matrices can be decomposed as:
% \begin{equation}
% Q =
% \begin{bmatrix}
% Q_{U} \\
% Q_{I}
% \end{bmatrix},
% \qquad
% K =
% \begin{bmatrix}
% K_{U} \\
% K_{I}
% \end{bmatrix}.
% \end{equation}
% To prevent U-side representations from attending to I-side information, 
% we introduce a binary attention mask $M \in \{0,1\}^{H \times H}$, where H is the attention head number. The masked attention is computed as:
% \begin{equation}
% \mathrm{Attn}_{UI}(X) =
% \left(\mathrm{softmax}\!\left(
%     \frac{QK^{\top}}{\sqrt{d}}\right) * M\right)V .
% \end{equation}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth,clip]{image/attention.jpeg}
%     \caption{Attention with UI Mask}
%     \label{fig:attention}
% \end{figure}






% \section{Experiment}
% \subsection{Experiment Settings}
% \subsubsection{Datasets and Environment}
% To comprehensively evaluate the effectiveness of our proposed method, we conduct offline experiments across multiple real-world business scenarios at ByteDance, including Douyin recommendation system, Hongguo recommendation, Chuanshanjia Ads and Qianchuan Ads. These tasks differ substantially in terms of user scale, content modality, feedback patterns, and data distributions, offering a comprehensive testbed to evaluate the model’s generalization ability and robustness across heterogeneous environments.

% All datasets are derived from real online interaction logs and user feedback signals. They contain hundreds to thousands of feature fields—including numerical, categorical, cross, and sequential features—spanning billions of user IDs and hundreds of millions of video or ad item IDs. Prior to model training, all features are transformed into sparse embedding representations to accommodate large-scale deep recommendation models. %This rich and diverse industrial dataset environment enables a systematic and rigorous evaluation of the proposed method.
% % \begin{table}[h]
% %     \centering
% %     \caption{Evaluation of methods on different industrial dataset and scenarios. U:I denotes the mixing ratio of user tokens to item tokens. “$\Delta$AUC” represents the improvement over the baseline model. Among these, an AUC decrement of 0.02-0.03\% has been verified through rigorous A/B testing to exert almost no impact on online performance. $\Delta$ Latency represents the serving latency improvement over the baseline model.}
% %     \label{tab:performance}
% %     \begin{tabular}{l|l l l l l l}
% %         \toprule
% %           Model & U:I & AUC  & $\Delta$ AUC & $\Delta$ Latency \\  
% %         \midrule
% %         \multirow{4}{*}{\textbf{DouYin Rec}} & base & 0.86143  & --& -- \\
% %         & 1:2 & 0.86145 & +0.00002   & --  \\
% %          & 1:1 & 0.86139 & -0.00004  & +20.0\% \\
% %          & 3:1 & 0.86130 & -0.00013  & -- \\
% %          \midrule
% %          \multirow{4}{*}{\textbf{HongGuo Rec}} & base & 0.90823  & --&-- \\
% %          & 1:1 & 0.90805 & -0.00018  & + 11.5\%\\
% %          & 5:3 & 0.90808 & -0.00015   & -- \\
% %          & 2:1 & 0.90790 & -0.00033  & --\\
% %          \midrule
% %           \multirow{3}{*}{\textbf{Chuanshanjia Ads}} & base & 0.88329  & --&-- \\
% %           & 1:1 & 0.88313 & -0.00016  & +12.7\%\\
% %          & 5:3 & 0.88303 & -0.00026  & --\\
% %          \midrule
% %            \multirow{2}{*}{\textbf{Qianchuan Ads}}& base & 0.84557 & -- & -- \\
% %          & 1:1 & 0.84533 & -0.00024  & +22.0\%\\
% %         \bottomrule
% %     \end{tabular}
% % \end{table}
% \begin{table}[h]
%     \centering
%     \caption{Evaluation of methods on different industrial dataset and scenarios. U:I denotes the mixing ratio of user tokens to item tokens. “$\Delta$AUC” represents the improvement over the baseline model. Among these, an AUC decrement of 0.02-0.03\% has been verified through rigorous A/B testing to exert almost no impact on online performance. $\Delta$ Latency represents the serving latency improvement over the baseline model.}
%     \label{tab:performance}
%     \begin{tabular}{l|l l l l l}
%         \toprule
%           Model & U:I   & $\Delta$AUC & $\Delta$Latency \\  
%         \midrule
%         \multirow{4}{*}{\textbf{Douyin Rec}} & base &  --& -- \\
%         & 1:2 &  +0.00002   & --  \\
%          & 1:1 & -0.00004  & +20.0\% \\
%          & 3:1 & -0.00013  & -- \\
%          \midrule
%          \multirow{4}{*}{\textbf{Hongguo Rec}} & base &  --&-- \\
%          & 1:1 & -0.00018  & + 11.5\%\\
%          & 5:3 & -0.00015   & -- \\
%          & 2:1 & -0.00033  & --\\
%          \midrule
%           \multirow{3}{*}{\textbf{Chuanshanjia Ads}} & base &  --&-- \\
%           & 1:1 & -0.00016  & +12.7\%\\
%          & 5:3 & -0.00026  & --\\
%          \midrule
%            \multirow{2}{*}{\textbf{Qianchuan Ads}}& base & -- & -- \\
%          & 1:1 & -0.00024  & +22.0\%\\
%         \bottomrule
%     \end{tabular}
% \end{table}


% \subsubsection{Baseline}
% We conduct our evaluations on the following four models: 
% \begin{enumerate}
%   \item \textbf{Douyin Rec}:  
%   We evaluate the ranking model in the Douyin recommendation system whose backbone is based on the RankMixer\cite{zhu2025rankmixer} architecture. The training samples follow the user-level format, allowing us to measure both training acceleration and inference acceleration.
%   \item \textbf{Hongguo Rec}: A short-video recommendation model used in the Hongguo platform, also built upon a RankMixer backbone. Since its training samples are in a standard instance-level format, we only evaluate inference acceleration.
%     \item \textbf{Chuanshanjia Ads}: A CTR prediction model deployed in ChuanShanJia, primarily serving off-site traffic, with a backbone composed of RankMixer layers. Similar to Hongguo, its training samples are standard instance-level, and therefore only inference acceleration can be measured.
%     \item {\textbf{Qianchuan Ads}}: An Ads CVR model in Douyin with a core architecture based on the RankMixer.
% \end{enumerate}

% \subsubsection{Evaluation Metrics}
% For model performance evaluation, we adopt the Area Under the ROC Curve (AUC) as the primary metric. AUC is widely used in large-scale recommendation and prediction tasks, as it effectively measures the model’s ability to distinguish between positive and negative samples and remains robust under imbalanced data distributions.

% \subsubsection{ Implementation Details}
% Since the RankMixer constitutes the core building block of these models, UI-seq is primarily applied to the RankMixer modules. During training, the same training protocol as the baseline is adopted, using large-scale industrial datasets to ensure a fair and consistent comparison.

% \subsection{Offline Evaluation}

% \subsubsection{AUC}

% Table \ref{tab:performance} reports the AUC performance of UI-Sep under different model settings and U:G token ratios. Overall, UI-Sep maintains highly stable predictive accuracy across all evaluated models. For the Douyin ranking model, AUC variations remain within ±1e-4 across different ratios, indicating that user–item separation introduces negligible impact on model effectiveness. Similar trends are observed in the HongGuo, ChuanShanJia, and Qianchuan models, where slight AUC fluctuations are consistently below 0.0003. These results demonstrate that the proposed separation and compensation mechanisms effectively retain model expressiveness while enabling computation reuse.

% \subsubsection{Different UI Token Ratios}
% We also investigate the effect of different U:G token mixing ratios on model performance. As shown in Table  \ref{tab:performance}, moderate ratios such as 1:1 or 1:2 consistently achieve a favorable balance between accuracy and efficiency. In the Douyin model, increasing the proportion of user tokens leads to marginal AUC changes while improving training throughput. However, excessively skewed ratios (e.g., 3:1) do not provide additional accuracy benefits and may introduce unnecessary redundancy. Similar observations hold for HongGuo and ChuanShanJia, suggesting that UI-Sep is robust across a range of token ratios, with balanced configurations offering the most stable trade-off between accuracy and computational gains.

% \begin{table}[t]
% \centering
% \caption{Relative training speedup of the Douyin Rec model under different U:I ratios.}
% \begin{tabular}{c c c}
% \hline
% Model & U:I & Training Speedup (\%) \\
% \hline
% RankMixer & --  & 0.0 \\
% \hline
% \multirow{3}{*}{RankMixer-v2} 
% & 1:2 & +5.50 \\
% & 1:1 & +8.60 \\
% & 3:1 & +14.8 \\
% \hline
% \end{tabular}
% \label{tab:douyin_speedup}
% \end{table}
% \subsubsection{Training Acceleration}
% Since the training samples in Douyin adopt the user-level format, we present the resulting training throughput speedup in Table~\ref{tab:douyin_speedup}. Increasing the U-side ratio leads to stronger acceleration, with an 8.6\% speedup observed at the 1:1 setting.
% \subsubsection{Latency}
% UI-Sep delivers consistent serving latency reductions across all evaluated models. In the Douyin production model, adopting a 1:1 UI ratio reduces serving latency corresponding to an 20\% improvement, while preserving comparable AUC. In addition to inference acceleration, Douyin also benefits from training throughput improvements, with throughput increasing from 1280k/s to 1390k/s under the 1:1 configuration. This gain arises because Douyin training samples follow the user-level-training format, which allows user-side computations to be shared across samples during training, enabling UI-Sep to reduce redundant computation on the user side.

% For HongGuo and ChuanShanJia, serving latency is still reduced by 11.5\% and 12.7\%, respectively. Notably, the large-scale 7B model in Qianchuan Ads achieves the largest latency reduction of 22.0\%, highlighting that the benefits of UI-Sep become more pronounced as model size and inference cost increase. Overall, these results demonstrate that UI-Sep effectively accelerates inference in all settings, and can additionally improve training efficiency when user-level aggregation is available.

% % where training samples are not organized in the ULT format, training throughput remains largely unchanged, while

% \subsection{Abation Study}
% To better understand the contribution of each component in our method, we perform a series of ablation studies. Specifically, we evaluate the impact of the Information Compensation module on AUC and examine how W8A16 quantization affects throughput.
% \subsubsection{Information Compensation}
% \begin{table}[h]
% \centering
% \caption{Ablation study on Information Compensation under different U:G ratios.}
% \begin{tabular}{lcc}
% \toprule
% \textbf{U:I Ratio} & \textbf{Info Compensation} & $\Delta$\textbf{AUC} \\
% \midrule
% 1:2 & N & +0.00\% \\
% 1:1 & N & -0.01\% \\
% 2:1 & N & -0.04\% \\
% 3:1 & N & -0.06\% \\
% \midrule
% 3:1 & Y & -0.02\% \\
% 5:1 & Y & -0.04\% \\
% \bottomrule
% \end{tabular}
% \label{tab:info_comp_ablation}
% \end{table}


% To further examine the role of Information Compensation, we conduct an ablation study across various U:I token ratios, as shown in Table~\ref{tab:info_comp_ablation}. Without the compensation mechanism, model performance deteriorates as the U-side proportion increases. The AUC drops from $-0.01\%$ at 1:1 to $-0.04\%$ at 2:1, and further to $-0.0\%$ at 3:1. This degradation suggests that the information obscured by UI separation masking becomes increasingly unrecoverable when the model allocates more capacity to the user-side tokens, and residual connections alone are insufficient to compensate for this loss.

% After enabling Information Compensation, however, the model exhibits notable improvements. At the 3:1 ratio, the AUC improves from $-0.06\%$ to $-0.02\%$, demonstrating a clear recovery of the masked information. Even at the highly imbalanced 5:1 ratio, the model maintains stable performance ($-0.04\%$) with compensation enabled. These findings indicate that the Information Compensation module effectively mitigates the information loss caused by UI masking and plays a crucial role in stabilizing model behavior under skewed U:G configurations. Overall, the ablation results validate that Information Compensation is a key component of our framework, especially when the model emphasizes the user-side representation.
% \begin{table}[h]
% \centering
% \caption{GEMM-level latency reduction after applying W8A16 on UI.}
% \begin{tabular}{lcc}
% \toprule
% \textbf{BS M N K}  & \textbf{UI + W8A16} \\
% \midrule
% (1,16, 1280, 2560)  & \textbf{-50.2\%} \\
% (1,16, 1280, 640) & \textbf{-40.0\%} \\
% (1,8, 1280, 2560)  & \textbf{-46.8\%} \\
% (1,8, 1280, 640)  & \textbf{-55.0 \%} \\
% \bottomrule
% \end{tabular}
% \label{tab:w8a16_ablation}
% \end{table}

% % \begin{table}[h]
% % \centering
% % \caption{GEMM-level latency comparison before and after applying W8A16.}
% % \begin{tabular}{lcc}
% % \toprule
% % \textbf{BS M N K} & \textbf{UI-only } & \textbf{UI + W8A16} \\
% % \midrule
% % (1,16, 1280, 2560)  & 203\,$\mu$s & \textbf{101\,$\mu$s} \\
% % (1,16, 1280, 640)  & 55\,$\mu$s & \textbf{23\,$\mu$s} \\
% % (1,8, 1280, 2560) & 124\,$\mu$s & \textbf{66\,$\mu$s} \\
% % (1,8, 1280, 640)  & 40\,$\mu$s & \textbf{18\,$\mu$s} \\
% % \bottomrule
% % \end{tabular}
% % \label{tab:w8a16_ablation}
% % \end{table}


% \subsubsection{W8A16}
% To further investigate the impact of W8A16 on operator-level performance, we conduct a GEMM-specific ablation study, as summarized in Table \ref{tab:w8a16_ablation}. Although UI-separation reduces FLOPs, its latency improvement remains limited because the execution is dominated by memory bandwidth rather than compute operations. By applying W8A16—an 8-bit weight-only quantization scheme—the memory bound is substantially reduced, leading to significant reductions in GEMM latency across U-side tested shapes.

% As shown in Table \ref{tab:w8a16_ablation} , W8A16 reduces GEMM-level latency by 40.0\%–55.0\% across all evaluated configurations.
% These gains highlight that weight loading, not computation, is the primary cost in memory-bound recommendation workloads, and that weight-only quantization provides an effective mechanism to alleviate this bottleneck. Importantly, because activations remain in 16-bit precision, the expressiveness and numerical stability of the forward computation are preserved.

% Overall, these results demonstrate that W8A16 provides substantial operator-level acceleration in memory-bound regimes, making it an essential component for realizing the practical benefits of UI-separation. The quantization overhead is negligible compared to the reduction in memory bandwidth, enabling significant latency improvements without sacrificing numerical stability.


% \begin{table}[h]
% \centering
% \caption{Online A/B Test Results on Douyin recommendation system: Key Behavioral Metrics (RankMixer-v2 vs. RankMixer-v1).}
% \label{tab:online_ab}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Category} & \textbf{Metric} & \textbf{Change}(\%)& \textbf{$p$-value} \\
% \midrule
% \multirow{1}{*}{Active Days} 
% & ValidSession/User (14d) & -0.0117& 0.46 \\
% \midrule
% \multirow{2}{*}{\shortstack{7-day Active\\ Users}}
% & FavouriteUser/User & -0.0069& 0.58 \\
% & LikeUser/User & +0.0012 & 0.87\\
% \midrule
% \multirow{2}{*}{\shortstack{7-day Video \\Interactions}}
% & share\_cnt\_7d/vv\_7d & +0.0621 & 0.28 \\
% & follow\_cnt\_7d/vv\_7d & -0.0206& 0.87 \\
% \midrule
% Latency&--&-20.0\% &--\\
% \midrule
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \centering
% \caption{Online A/B Test Results on ChuanShanJia : Key Behavioral Metrics (RankMixer-v2 vs. RankMixer-v1)}
% \label{tab:ChuanShanJia}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Metric} & \textbf{Change} (\%) & \textbf{$p$-value} \\
% \midrule
% Cost            & -0.1143 & 0.45 \\
% Rank Advv       & -0.1322 & 0.42 \\
% Advv (Overall)  & -0.2042 & 0.32 \\
% \midrule
% Latency & -12.7\% &-- \\
% \bottomrule
% \end{tabular}
% \end{table}


% \subsection{Online A/B Tests}
% We conducted large-scale online A/B experiments to assess the real-world impact of the proposed method by comparing RankMixer-v2 against RankMixer-v1 on both the Douyin recommendation system and the ChuanShanJia advertising platform.

% As shown in Table~\ref{tab:online_ab}, key user behavioral metrics on the Douyin recommendation system—including user activeness, short-term action behaviors, and video interaction signals—exhibit only marginal relative changes, with absolute variations generally within 0.1\%. Importantly, all observed changes, whether positive or negative, are associated with high $p$-values, indicating that none of the differences reach statistical significance. These results suggest that the proposed method does not materially affect core user engagement behaviors in the recommendation system.

% Similarly, the online results on the ChuanShanJia platform (Table~\ref{tab:ChuanShanJia}) show slight decreases in cost and Advv-related metrics, including Rank Advv and overall Advv. However, the magnitudes of these changes remain small (below 0.25\%), and all corresponding $p$-values are well above conventional significance thresholds. Therefore, these variations should be interpreted as statistically insignificant fluctuations rather than systematic performance shifts.

% Overall, across both platforms, no statistically significant improvements or decrements are observed. The consistent absence of significant changes indicates that the proposed approach maintains stable online performance, preserving both user engagement and monetization efficiency. 




% \section{Conclusion}

% This paper addresses a key efficiency bottleneck in dense recommender models, where deep user–item feature entanglement prevents reuse of user-side computation and leads to high inference cost. We propose User–Item Separation (UI-Sep), a general framework that enables user-side computation reuse in dense interaction architectures. UI-Sep introduces a masking mechanism to disentangle user–item information flows, an information compensation strategy to preserve model expressiveness, and W8A16 quantization to alleviate memory bottlenecks exposed after reducing user-side FLOPs.

% Extensive offline evaluations and large-scale online A/B tests demonstrate that UI-Sep achieves significant inference acceleration while maintaining stable accuracy and healthy online metrics. In a production deployment within Douyin’s recommendation system, UI-Sep reduces inference latency by up to 18\% without adverse impact on user behavior. Overall, UI-Sep provides a practical and effective solution for scaling dense recommender models in real-world industrial settings.

% \bibliographystyle{ACM-Reference-Format}
% \bibliography{ref.bib}

% \end{document}
% \endinput
% %%
% %% End of file `sample-sigconf.tex'.

